Eversion-based robots can enable safe access,steering and endoscopic imaging within the spinal subarachnoid space

Safe navigation within the spinal subarachnoid space is constrained by its narrow, compliant, and delicate anatomy. Conventional catheters and continuum robots rely on proximal pushing, generating friction and shear along the tissue device interface that limit distal controllability and increase the risk of neural injury. Here, we present a 2 mm diameter eversion-growing robotic platform that enables friction minimised extension and steering within the human spinal subarachnoid space, validated through computational modelling, phantom experiments, and intact human cadaver studies. The robot integrates a miniature endoscope for real time intrathecal visualisation and advances by pressure driven tip eversion, localising motion to the distal tip while minimising translational sliding of the deployed body. Phantom experiments demonstrated reductions of 65.2% in mean interaction force and 48.0% in peak interaction force compared with matched push-based insertion. Physics based modelling showed that eversion based growth redistributed tissue loading, reducing local stress concentrations and interfacial shear relative to conventional insertion. In an intact human cadaver, the system achieved 150 mm of controlled intrathecal extension with concurrent fluoroscopic and endoscopic visualisation, providing access across multiple vertebral levels from a standard lumbar entry point. Postprocedural laminectomy and durotomy revealed no observable macroscopic disruption of the dura mater or surrounding neural structures. These results provide the first mechanically characterised and multimodally validated demonstration of eversion-based robotic navigation in intact human spinal anatomy, establishing a quantitative and procedural foundation for future intrathecal interventions. Further validation in larger anatomical cohorts and under physiological conditions will be required before clinical translation.

==> removedText.tex <==
%Therapeutic Approaches
Emerging therapeutic approaches, including gene-based therapies, neuromodulation, bioelectronic medicine, and cell-based regenerative therapies, have been proposed and explored, demonstrating clinical effectiveness targeting ND diseases \cite{aybek2022diagnosis}. 
Recent advancements in gene-based therapies have expanded the therapeutic approaches to the treatment of ND diseases. Via various delivery vehicles, the genetic material aims to induce gene silencing or gene editing, leading to the desired expression of a therapeutic, function-restorative protein as therapeutic agents \cite{ling2023aav}.
Different types and shapes of nanomaterials have been widely explored for the treatment of neurological disorders, including quantum dots, dendrimers, metallic nanoparticles, polymeric nanoparticles, carbon nanotubes, liposomes, and micelles, demonstrating unique characteristics \cite{waris2022applications}. 
By harnessing the regenerative potential of stem cells to restore damaged neural tissue and circuitry, the stem cell therapies hold transformative potential for multiple NDs, and promising results have been reported in animal models and clinical trials at different stages\cite{rahimi2024stem,temple2023advancing}.

%Brain Blood Barriers
As a vulnerable and complex system, the central nervous system introduces complications and challenges in the diagnosis and treatment of ND diseases. Some particular structures, known as the brain blood barriers, regulate the molecular exchange between the blood and the brain, and create complications for therapeutic intervention. The brain-blood-barriers are made up of glial cells and endothelial cells, administering the therapeutic agents' access to the central nervous system \cite{daneman2015blood}.

%Spinal Subrachanoid Space
Therapies and diagnostics targeting the central nervous system increasingly rely on direct access to cerebrospinal fluid spaces, bypassing the limitations imposed by the blood–brain barrier. In particular, the spinal subarachnoid space has emerged as a clinically relevant pathway for intrathecal drug delivery, neuromodulation, and diagnostic interrogation. However, this space is anatomically narrow, compliant, and densely surrounded by critical neural structures, rendering safe navigation highly challenging.


This property has enabled safe navigation in fragile and confined environments \cite{wooten2018exploration,del2024growing,,wu2025soft} and has motivated exploration of medical applications \cite{oyejide2025miniaturized}, including endovascular intervention \cite{li2021vine}, mammary ducts inspection\cite{berthet2021mammobot,wu2023towards,wu2023vision}, colonoscopy \cite{borvorntanajanya2024model,shi2025design}, and transoral and endoluminal airway procedures \cite{xu2024novel,hwee2021everting}. 
Despite these advantages, eversion-growing robots have not been previously demonstrated within the spinal subarachnoid space or validated in human tissue. The anatomical constraints, sterility requirements, and need for integrated sensing and imaging pose significant challenges that have, until now, prevented translation of this paradigm to spinal interventions.
